Nonparametric Bayesian Mixed-effect Model: a Sparse Gaussian Process Approach

Multi-task learning models using Gaussian processes (GP) have been developed and successfully applied in various applications. The main difficulty with this approach is the computational cost of inference using the union of examples from all tasks. Therefore sparse solutions, that avoid using the entire data directly and instead use a set of informative "representatives" are desirable. The paper investigates this problem for the grouped mixed-effect GP model where each individual response is given by a fixed-effect, taken from one of a set of unknown groups, plus a random individual effect function that captures variations among individuals. Such models have been widely used in previous work but no sparse solutions have been developed. The paper presents the first sparse solution for such problems, showing how the sparse approximation can be obtained by maximizing a variational lower bound on the marginal likelihood, generalizing ideas from single-task Gaussian processes to handle the mixed-effect model as well as grouping. Experiments using artificial and real data validate the approach showing that it can recover the performance of inference with the full sample, that it outperforms baseline methods, and that it outperforms state of the art sparse solutions for other multi-task GP formulations.

==> longtexfiles/prelim.tex <==

\section{Preliminaries}

This section provides the technical background on GPs, sparse GPs,
and the mixed effect model for multi-task learning with GPs.

\subsection{Gaussian Processes and Sparse Solutions}

A GP specifies a distribution over functions, so that every finite sample of
function values is normally distributed.
In single task learning using GP, we collect a training set $\D =
\{(\x_i,y_i)\}, i = 1,2,\cdots, N$  where we assume $f$ to be a zero-mean GP with covariance function $K$,
\begin{equation}
  y_i = f(\x_i) + \epsilon_i, \qquad \mbox{ and } \qquad \epsilon_i\sim\mathcal{N}(0,\sigma^2).
\end{equation}
Let $\y=[y_1,\cdots,y_n]^\T, \quad \f=[f(\x_1),\cdots,
f(\x_n)]^\T$ be the observations and the corresponding vector of the
latent \emph{training set} function values. The predictive
distribution for a new sample point $\x^*$ is given by
\begin{displaymath}
  \begin{split}
    &\Pr(f(\x_*)|\x_*,\D)= \int \Pr(f(\x_*)|\x_*, f)\Pr(f|\D)df\\
    &= \mathcal{N}\bigg(\mathbf{k}(\x_*)^\T(\sigma^2\mathbb{I}+\fK)^{-1}\y, \\
    &\qquad\quad\fK(\x_*, \x_*) -\mathbf{k}(\x_*)^\T(\sigma^2\mathbb{I}+\fK)^{-1}\mathbf{k}(\x_*)\bigg)
  \end{split}
\end{displaymath}
where $\mathbf{k}(\x_*) = [K(\x_1,\x_*),\cdots,K(\x_N,\x_*)]^\T$.
This is the standard formulation of GP regression which we use repeatedly
below. We also use standard results on marginalization and conditioning of
Gaussian distributions \cite{rasmussen2005gaussian,bishop2006pattern}.
Computing the predictive distribution requires inverting the
kernel matrix, with a cost of $O(N^3)$, which is too high for large scale
problems.

To reduce the computational cost,
several sparse GP approaches have been proposed
\cite{rasmussen2005gaussian,Seeger03,Snelson06,titsias2008variational}.
In general, these
methods approximate the GP with a small number $m \ll N$ of support
variables and
perform inference using this subset and the corresponding function values $\f_m$.
% should be ^3 at least during learning but once k_mm^-1 is available
% we get Nn^2
%reduces the time complexity to $O(Nm^2)$.
Different approaches
differ in how they choose the
support variables and the simplest approach is to choose a random subset of
the given data points.
Recently, Titsias \cite{titsias2008variational} introduced
a sparse method based on variational inference
using a set $\mathcal{X}_m$ of
inducing samples, which are independent from the training
points.
% and their values $\f_m$.
In this approach, the sample points $\mathcal{X}_m$ are chosen to maximize
a variational lower bound on the marginal likelihood, therefore providing a
clear methodology for the choice of the support set.
%Experiments in \cite{titsias2008variational} showed that this approach
%significantly outperforms previous sparse formulations of GPs.
In this paper we extend this approach to the multi-task setting.

%Using this method,
%if $\f_m \sim
%\mathcal{N}(\mu, A)$, then the predictive distribution
%is
%%~\cite{unknown}
%\begin{equation}
%  \begin{split}
%    \Pr(f(\x_*)|\x_*,\D)&= \mathcal{N}\bigg(\pk_m(\x_*)^\T\fK_{mm}^{-1}\y,\\
%    &\quad   \fK(\x_*, \x_*) -
%    \pk_m(\x_*)^\T\fK_{mm}^{-1}\pk_m(\x_*) +
%    \sigma^2\pk_m(x_*)^\T\fK_{mm}^{-1}A\fK_{mm}^{-1}\pk_m(\x_*)\bigg).
%  \end{split}
%\end{equation}


%In~\cite{titsias2008variational}, the author introduce a small set of $m$ auxiliary inducing variables $\f_m$ evaluated at the pseudo-inputs $\mathcal{X}_m$ which are independent from the training points. Therefore given any finite set of function points $\z$, we have
%\begin{displaymath}
%\begin{split}
%  \Pr(\z|\y) &= \int\Pr(\z, \f, \f_m|\y)d\f d\f_m\\
%  &= \int\Pr(\z| \f, \f_m)\Pr(\f|\f_m, \y)\Pr(\f_m|\y)d\f d\f_m\\
%\end{split}
%\end{displaymath}
%From the previous equation, we can see that the idea is to find an inducing set based on which we can approximate $\z$ as well as $\y$ well with much less computational cost. If $\f_m$ is assumed to be a sufficient statistic for the parameter $\f$ in the sense that $\z$ and $\f$ are independent given $\f_m$, we have
%\begin{equation}
%\label{eqn:qz}
%\begin{split}
%  \Pr(\z|\y) &= \int\Pr(\z|\f_m)\Pr(\f|\f_m)\phi(\f_m) d\f d\f_m\\
%  &= \int\Pr(\z|\f_m)\phi(\f_m) d\f_m\\
%\end{split}
%\end{equation}
%where $\phi(\f_m) = \Pr(\f_m|\y)$. We can see that computing Eq.~(\ref{eqn:qz}) only need $O(nm^2)$ time. The problem is how can we choose the variational $\phi(\f_m)$. To approximate $\Pr(\f,\f_m|\y) = \Pr(\f|\f_m)\Pr(\f_m|\y)$, the author choose the variation distribution $\phi(\f_m)$ such that it minimizes the KL divergence:
%\begin{equation}
%\label{eqn:KL}
%  \text{KL}(q(\f,\f_m)\|p(\f,\f_m|\y)) = \int q(\f, \f_m)\log\frac{q(\f,\f_m)}{p(\f,\f_m|y)}d\f d\f_m
%\end{equation}
%where $q(\f, \f_m) = \Pr(\f|\f_m)\phi(\f_m)$.

